Can RAG-Based QA Stay Neutral? Selective Amplification of Informational Bias over Politically Framed Sources

Informational bias arises when media articles selectively include or emphasize facts to shape readers' interpretations. This poses risks for retrieval-augmented generation (RAG) systems: when retrieved articles present divergent political leanings, it remains unclear whether RAG systems exhibit selective bias by inheriting or amplifying informationally biased facts from particular sources. We introduce PoliFrameQA, a fact-level benchmark for analyzing informational bias in RAG-based question answering. Each question is paired with articles from different political leanings. For every leaning we obtain a reference answer grounded in that leaning's article alone, decompose it into atomic facts, and annotate which of those facts reflect informationally biased framing. To scale annotation, we propose a two-stage pipeline for identifying informationally biased facts. Experiments on RAG systems with open- and closed-source LLMs show that these systems inherit informational bias and selectively amplify bias from certain political leanings, while general bias mitigation methods yield no Pareto improvements in the coverage-bias trade-off.

==> sections/15_experiment_safe_prev_version.tex <==
\section{Experiments and Results}
\label{sec:exp}

\subsection{Experimental Setup}
\label{sec:exp-setup}

%We evaluate five instruction-tuned LLMs---\textsc{GPT-4o-mini}, \textsc{LLaMA-2-7B-Chat}, \textsc{Qwen2-7B-Instruct}, \textsc{TxGemma-9B-Chat}, \textsc{DeepSeek-7B-Chat}---each prompted with $\mathcal{Q}$ and the concatenated triplet to produce the all-sides answer $\mathcal{A}_{\text{all}}$, under three settings: \textbf{vanilla} (the unmodified triplet; \S\ref{sec:exp-vanilla}), \textbf{debiasing} (four mitigation methods; \S\ref{sec:exp-debias}), and a \textbf{noisy-context} ablation (\S\ref{sec:exp-noisy}).
%Every answer is scored against the same reference bias landscape---the shared facts $\mathcal{F}_{\text{share}}$ and the per-stance biased ($f_{\text{bias}}^{k}$) and neutral ($f_{\text{unb}}^{k}\!=\!f_{\text{uni}}^{k}\setminus f_{\text{bias}}^{k}$) partitions defined in Sections~\ref{sec:data-task-form} and~\ref{subsec:metrics}---produced once by the pipeline of Section~\ref{sec:data-data-collection}.
%Because \textsc{GPT-4o-mini} grounds this landscape, its own scores are reported for completeness but excluded from rankings.
%Vanilla baselines use the full test set ($n\!=\!1907$); the debiasing and noisy settings use a fixed $n\!=\!500$ subsample, which agrees with the full set to within $1.8$ percentage points (pp) on \textsc{LLaMA-2-7B-Chat}.
%Additional experimental settings including decoding details and \textsc{Gemma-3-27B-it} fact decomposer are provided in Appendix~\ref{app:exp-setup-details}.

We evaluate five instruction-tuned LLMs: \textsc{GPT-4o-mini}, \textsc{LLaMA-2-7B-Chat}, \textsc{Qwen2-7B-Instruct}, \textsc{TxGemma-9B-Chat}, and \textsc{DeepSeek-7B-Chat}. Each model receives $\mathcal{Q}$ and the concatenated left-/center-/right-leaning article triplet $\mathcal{D}=\{D^{L},D^{C},D^{R}\}$, and generates the all-sides answer $\mathcal{A}_{\mathrm{all}}$. Because our evaluation requires only black-box generation, the pool can pair a widely deployed closed-weight model with open-weight models in the 7--9B class; Section~\ref{sec:exp-scale} extends it with larger and more recent models.


We consider three settings. \textbf{Vanilla} uses the original triplet to test whether RAG systems inherit informational bias from multi-perspective evidence. \textbf{Debiasing} applies four mitigation methods to test whether answer-level bias can be reduced without sacrificing coverage. \textbf{Noisy context} prepends an off-triplet web-retrieved chunk to test whether the evaluation remains stable when evidence is less curated.

%All answers are scored against the same reference bias landscape: shared facts $\mathcal{F}_{\mathrm{share}}$, stance-specific biased facts $\mathcal{F}_{\mathrm{bias}}^{k}$, and stance-specific neutral facts $\mathcal{F}_{\mathrm{unb}}^{k}=\mathcal{F}_{\mathrm{uni}}^{k}\setminus\mathcal{F}_{\mathrm{bias}}^{k}$, as defined in Sections~\ref{sec:data-task-form} and~\ref{subsec:metrics}. This landscape is produced once by the annotation pipeline in Section~\ref{sec:data-data-collection}. Since \textsc{GPT-4o-mini} helps construct the reference landscape, we report its scores for completeness but exclude it from rankings. Vanilla baselines use the full test set ($n\!=\!1907$); debiasing and noisy-context experiments use a fixed $n\!=\!500$ subsample, whose \textsc{LLaMA-2-7B} scores differ from the full set by at most $1.8$ percentage points\weicomment{Why? How can you justify this cleanly?}. Decoding details and the \textsc{Gemma-3-27B-it} fact decomposer are in Appendix~\ref{app:exp-setup-details}.

All answers are scored against a fixed reference landscape produced by the annotation pipeline: shared facts $\mathcal{F}_{\mathrm{share}}$, stance-specific biased facts $\mathcal{F}_{\mathrm{bias}}^{k}$, and stance-specific neutral facts $\mathcal{F}_{\mathrm{unb}}^{k}$ (Sections~\ref{sec:data-task-form} and~\ref{subsec:metrics}). Since \textsc{GPT-4o-mini} contributes to this landscape, we report its scores only for completeness and exclude it from rankings. Vanilla baselines use the full test set ($n\!=\!1907$); debiasing and noisy-context experiments use a fixed $n\!=\!500$ subsample (the first $500$ instances in the canonical benchmark order). We verify representativeness by recomputing \textsc{LLaMA-2-7B}'s vanilla scores on this subset: $\mathrm{BiasRatio}$ shifts by $0.3$ percentage points (pp), $\mathrm{Coverage}$ by $2.8$~pp, and the per-stance $\mathrm{SBias}^{k}$ by at most $4.8$~pp, leaving the model's operating point qualitatively unchanged. Decoding details and the \textsc{Gemma-3-27B-it} fact decomposer are in Appendix~\ref{app:exp-setup-details}.

\subsection{Vanilla RAG Baselines}
\label{sec:exp-vanilla}

%\paragraph{\rm \textbf{RQ1 \& RQ2}: Do RAG systems inherit informational bias in their generated all-sides answers (RQ1), and are they more susceptible to, or more likely to amplify, bias associated with particular political stances (RQ2)?}

%We quantify how the five models trade information retention against bias inheritance when supplied with the unmodified evidence triplet $(c_l,c_c,c_r)$.
%Figure~\ref{fig:pareto} renders the $(\mathrm{Coverage},\mathrm{BiasRatio})$ plane and Figure~\ref{fig:sbias_vanilla} visualizes the per-stance leakage; the underlying numerics are reported in Table~\ref{tab:baseline} in Appendix~\ref{app:vanilla-numbers}.

\paragraph{\rm \textbf{RQ1 \& RQ2}: Do RAG systems inherit informational bias, and is this inheritance stance-selective?}

Figure~\ref{fig:pareto} shows the $\mathrm{Coverage}$--$\mathrm{BiasRatio}$ trade-off, Figure~\ref{fig:sbias_vanilla} reports per-stance leakage, and full numbers are in Table~\ref{tab:baseline} in Appendix~\ref{app:vanilla-numbers}.

\begin{figure}[t]
\centering
\safeincludegraphics[width=\linewidth]{pic/fig_pareto_vanilla.pdf}
%\caption{$(\mathrm{Coverage},\mathrm{BiasRatio})$ plane for the five vanilla baselines on \our ($n\!=\!1907$).
%The upper-left region (high $\mathrm{Coverage}$, low $\mathrm{BiasRatio}$) is the desired regime.
%No model dominates: \textsc{GPT-4o-mini} maximizes information retention at the cost of high bias density, \textsc{LLaMA-2-7B} occupies the opposite corner, and \textsc{TxGemma-9B} attains the lowest per-stance leakage at moderate $\mathrm{Coverage}$.}
\caption{$(\mathrm{Coverage},\mathrm{BiasRatio})$ plane for vanilla baselines on \our ($n\!=\!1907$). The desired region is upper-left: high coverage and low bias.}
\label{fig:pareto}
\end{figure}

%\paragraph{Vanilla models occupy distinct, non-dominated points on the Coverage--BiasRatio plane.}
%Figure~\ref{fig:pareto} shows that the four non-reference models form a Pareto front rather than collapsing onto a single operating point.
%\textsc{GPT-4o-mini} attains the highest $\mathrm{Coverage}$ ($.587$) but also the highest bias on every measure (full numbers in Appendix~\ref{app:vanilla-numbers}).
%\textsc{LLaMA-2-7B} occupies the opposite corner: it minimizes $\mathrm{BiasRatio}$ ($.076$) but loses $11.1$~pp of $\mathrm{Coverage}$ relative to \textsc{GPT-4o-mini}.
%\textsc{TxGemma-9B} dominates on stance-conditional leakage---its per-stance scores $\mathrm{SBias}^{l}\!=\!.487$, $\mathrm{SBias}^{r}\!=\!.512$, $\mathrm{SBias}^{c}\!=\!.485$ are uniformly the lowest among the non-reference baselines---at moderate $\mathrm{Coverage}$ ($.542$).
%\textsc{Qwen2-7B} and \textsc{DeepSeek-7B} lie in the interior of the front.
%The fact that no single model dominates motivates our multi-metric reporting: $\mathrm{Coverage}$, $\mathrm{BiasRatio}$, and the per-stance $\mathrm{SBias}^{k}$ each rank the models differently.

\paragraph{Models form a non-dominated Coverage--BiasRatio frontier.}
Figure~\ref{fig:pareto} shows that no model is uniformly best. \textsc{GPT-4o-mini} achieves the highest $\mathrm{Coverage}$ ($.587$) but also the highest bias. \textsc{LLaMA-2-7B} minimizes $\mathrm{BiasRatio}$ ($.076$) but loses $11.1$~pp of $\mathrm{Coverage}$ relative to \textsc{GPT-4o-mini}. \textsc{TxGemma-9B} has the lowest per-stance leakage among non-reference models ($\mathrm{SBias}^{L}\!=\!.487$, $\mathrm{SBias}^{R}\!=\!.512$, $\mathrm{SBias}^{C}\!=\!.485$) at moderate $\mathrm{Coverage}$ ($.542$), while \textsc{Qwen2-7B} and \textsc{DeepSeek-7B} lie inside the front. This confirms the need to report $\mathrm{Coverage}$, $\mathrm{BiasRatio}$, and $\mathrm{SBias}^{k}$ jointly, since they capture different aspects of answer quality and bias.

\begin{figure}[t]
\centering
\safeincludegraphics[width=\linewidth]{pic/fig_sbias_vanilla.pdf}
%\caption{Per-stance selective bias $\mathrm{SBias}^{l}$, $\mathrm{SBias}^{r}$, $\mathrm{SBias}^{c}$ for the four non-reference vanilla baselines on \our ($n\!=\!1907$).
%For every model the center bar is the shortest: stance bias from the center-aligned source is the least likely to surface in the all-sides answer.
%\textsc{TxGemma-9B} also exhibits the smallest gap between $\mathrm{SBias}^{l}$ and $\mathrm{SBias}^{r}$, i.e.\ the most balanced leakage profile.
% \xdcomment{Adjust the size of numbers above the bar to avoid the overlap.}
%}
\caption{Per-stance selective bias for non-reference vanilla baselines on \our ($n\!=\!1907$). $\mathrm{SBias}^{R}$ exceeds $\mathrm{SBias}^{C}$ for every model: center-aligned biased facts are consistently under-amplified relative to right-aligned ones.}
\label{fig:sbias_vanilla}
\end{figure}

%\paragraph{Stance-conditional bias inheritance is structurally asymmetric.}
%Across every non-reference model in Figure~\ref{fig:sbias_vanilla}, $\mathrm{SBias}^{l}\!>\!\mathrm{SBias}^{c}$ and $\mathrm{SBias}^{r}\!>\!\mathrm{SBias}^{c}$.
%The $\mathrm{SBias}^{r}\!-\!\mathrm{SBias}^{c}$ gap ranges from $+1.8$~pp (\textsc{DeepSeek-7B}) to $+3.1$~pp (\textsc{LLaMA-2-7B}), while $\mathrm{SBias}^{l}\!-\!\mathrm{SBias}^{c}$ ranges from $-1.3$ to $+4.1$~pp.
%Center-aligned bias facts are therefore systematically the least likely to reappear in $\mathcal{A}_{\text{all}}$, mirroring the per-stance $\mathrm{BiasRate}$ asymmetry observed in the article triplets themselves.
%The plausible interpretation is that partisan information which all three sources could justify reads as ``triangulated'' to the model and is amplified less than information unique to a strong-stance source---a structural effect of selective amplification rather than a uniform bias floor.

\paragraph{Bias inheritance is stance-asymmetric.}
Across all non-reference models, the gap $\mathrm{SBias}^{R}-\mathrm{SBias}^{C}$ is positive, ranging from $+0.9$ to $+3.1$~pp, while $\mathrm{SBias}^{L}-\mathrm{SBias}^{C}$ ranges from $-1.3$ to $+4.1$~pp. Center-aligned biased facts are thus consistently under-amplified relative to right-aligned ones, and for two of the four models they are the least reproduced of all three stances.

%\paragraph{Low $\bm{\mathrm{BiasRatio}}$ can mask suppressed output, not filtered bias.}
%\textsc{LLaMA-2-7B}'s low $\mathrm{BiasRatio}$ co-occurs with the lowest $\mathrm{Coverage}$, while its per-stance leakage rates ($\mathrm{SBias}^{l}\!=\!.552$, $\mathrm{SBias}^{r}\!=\!.596$, $\mathrm{SBias}^{c}\!=\!.565$) are similar to mid-Coverage models.
%This pattern is consistent with \textsc{LLaMA-2-7B} reducing bias density by producing fewer atomic facts overall---both biased and unbiased---rather than by selectively filtering partisan content: the bias inheritance \emph{rate} (Eq.~\ref{eq:selective-bias}) is unchanged while the denominator of $\mathrm{BiasRatio}$ (Eq.~\ref{eq:bias-ratio}) shrinks.
%Reading $\mathrm{Coverage}$, $\mathrm{BiasRatio}$ and the per-stance $\mathrm{SBias}^{k}$ jointly is essential to distinguish such output shrinkage from genuine debiasing, a point we return to when analyzing debiasing methods below.

\paragraph{Low BiasRatio can reflect shorter answers rather than better filtering.}
\textsc{LLaMA-2-7B}'s low $\mathrm{BiasRatio}$ coincides with the lowest $\mathrm{Coverage}$, while its per-stance leakage ($\mathrm{SBias}^{L}\!=\!.552$, $\mathrm{SBias}^{R}\!=\!.596$, $\mathrm{SBias}^{C}\!=\!.565$) remains comparable to mid-coverage models. This indicates that its lower bias density is driven mainly by producing fewer facts overall, rather than selectively filtering biased ones.

%\paragraph{Finding.}
%Vanilla RAG-based QA systems do inherit informational bias from their evidence (\textbf{RQ1}): every benchmarked model leaks a non-trivial share of partisan facts into $\mathcal{A}_{\text{all}}$ ($\mathrm{BiasRatio}\!\in\![.076,.113]$, $\mathrm{SBias}^{k}\!\in\![.485,.677]$), and they do so \emph{selectively} (\textbf{RQ2}): center-aligned bias facts are systematically the least likely to be reproduced in $\mathcal{A}_{\text{all}}$ on every model, and individual models show distinct stance-conditional leakage profiles rather than a uniform bias floor.
%The trade-off across models is structured: closed-weight \textsc{GPT-4o-mini} favors information retention at the cost of high bias, while smaller open-weight models reduce bias density either by suppressing output (\textsc{LLaMA-2-7B}) or by hitting balanced operating points (\textsc{TxGemma-9B}, \textsc{DeepSeek-7B}).

\paragraph{Takeaway.}
Vanilla RAG systems inherit informational bias from retrieved evidence (\textbf{RQ1}) and do so stance-selectively (\textbf{RQ2}). Every model leaks a non-trivial share of biased facts into $\mathcal{A}_{\mathrm{all}}$ ($\mathrm{BiasRatio}\!\in\![.076,.113]$, $\mathrm{SBias}^{k}\!\in\![.485,.677]$), while in this pool center-aligned biased facts are consistently under-amplified relative to right-aligned ones. The trade-off is structured: \textsc{GPT-4o-mini} favors coverage at the cost of higher bias, whereas smaller open-weight models reduce bias density either by shortening answers or by occupying more balanced operating points.

\subsection{Debiasing Interventions}
\label{sec:exp-debias}

%\paragraph{\rm \textbf{RQ3}: Can common mitigation strategies reduce informational bias in all-sides answers?}

%To answer RQ3, we compare two prompt-side and two preference-alignment methods on \textsc{LLaMA-2-7B} and \textsc{Qwen2-7B}, the two open-weight workhorse models in our pool; \textsc{GPT-4o-mini} is excluded because it grounds the reference landscape.

%\paragraph{Prompt-side methods.}
%We adapt two strategies from \citet{lin-etal-2025-investigating} that intervene at inference time without modifying parameters.
%\textbf{Bias Label Explanation (BLE)} prepends explicit definitions of left-leaning, right-leaning, and center reporting to the system prompt, together with a final instruction to ``produce a balanced, unbiased answer that does not selectively emphasize facts aligned with any single political perspective.''
%\textbf{Debiasing Statement (DS)}, following \citet{ganguli2023capacity}, prepends a single short instruction asking the model to remain politically neutral, avoid loaded language, and present facts in a balanced manner.
%DS is the minimal-intervention counterpart to BLE.

%\paragraph{Preference-alignment methods.}
%We additionally evaluate two methods that fine-tune the model's weights using bias-graded preference data.
%\textbf{DPO}~\citep{rafailov2023dpo} forms preference pairs from our baseline pool in which the chosen response is the all-sides answer with lower stance-conditional leakage (smaller per-stance $\mathrm{SBias}^{k}$ summed over $k$) and the rejected response is the higher-leakage alternative, then optimizes the policy directly on these pairs without a separate reward model.
%\textbf{RLHF (PPO)}~\citep{rlhf} trains a reward model on the same preference pairs and updates the policy with PPO under a KL constraint against the supervised initialization, encouraging less stance-conditional leakage while preserving fluency.
%RLHF is applied only to \textsc{LLaMA-2-7B} due to compute budget; the remaining seven (method, model) combinations are reported.

\paragraph{\rm \textbf{RQ3}: Can common mitigation strategies reduce informational bias in all-sides answers?}

To answer RQ3, we evaluate four mitigation methods on \textsc{LLaMA-2-7B} and \textsc{Qwen2-7B}, the two open-weight models in our pool. \textsc{GPT-4o-mini} is excluded because it is used to construct the reference landscape. In contrast to evaluation, which needs only black-box access, preference alignment requires open weights and gradient access, so our compute budget restricts this line to the 7B scale. The methods cover two intervention types. First, we test two prompt-side methods that modify only the inference prompt. \textbf{Bias Label Explanation (BLE)} adapts \citet{lin-etal-2025-investigating} by adding definitions of left-, center-, and right-leaning reporting, followed by an instruction to produce a balanced answer that does not selectively emphasize any political perspective. \textbf{Debiasing Statement (DS)}, following \citet{ganguli2023capacity}, adds a shorter neutrality instruction asking the model to avoid loaded language and present facts evenly. Second, we test two preference-alignment methods using bias-graded preference pairs. \textbf{DPO}~\citep{rafailov2023dpo} chooses the answer with lower summed $\mathrm{SBias}^{k}$ as preferred and directly optimizes on these pairs. \textbf{RLHF (PPO)}~\citep{rlhf} trains a reward model on the same pairs and updates the policy with PPO under a KL constraint. RLHF is applied only to \textsc{LLaMA-2-7B} due to compute budget.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.5pt}
\scalebox{0.78}{
\begin{tabular}{@{}ll c c ccc@{}}
\toprule
\textbf{Model} & \textbf{Method} & $\mathrm{Cov.}\!\uparrow$ & $\mathrm{BR}\!\downarrow$
& $\mathrm{SB}^{L}\!\downarrow$ & $\mathrm{SB}^{R}\!\downarrow$ & $\mathrm{SB}^{C}\!\downarrow$ \\
\midrule
\multirow{5}{*}{\textsc{LLaMA}}
 & Vanilla & \textbf{.447} & .079          & \textbf{.512} & .579          & \textbf{.517} \\
 & BLE     & .437          & .070          & .590          & \textbf{.552} & .526          \\
 & DS      & .437          & .067          & .589          & .586          & .553          \\
 & RLHF    & .404          & .064          & .577          & .623          & .667          \\
 & DPO     & .228          & \textbf{.026} & .574          & .609          & .627          \\
\midrule
\multirow{4}{*}{\textsc{Qwen2}}
 & Vanilla & \textbf{.540} & .100          & .598          & .596          & .610          \\
 & BLE     & .448          & .071          & \textbf{.578} & .576          & .564          \\
 & DS      & .428          & .067          & .620          & \textbf{.572} & \textbf{.555} \\
 & DPO     & .206          & \textbf{.024} & .635          & .655          & .692          \\
\bottomrule
\end{tabular}}
%\caption{Debiasing methods on \our.
%Debiasing rows are evaluated on a fixed $n\!=\!500$ subsample; vanilla rows repeat Appendix~\ref{app:vanilla-numbers} (Table~\ref{tab:baseline}) for reference ($n\!=\!1907$; the $+1.8$~pp $\mathrm{Coverage}$ scale shift between $n\!=\!500$ and $n\!=\!1907$ is small relative to the debiasing effects discussed).
%\textbf{Bold}: best per column within each model section ($\uparrow$ for $\mathrm{Coverage}$, $\downarrow$ for the others).
%RLHF is applied only to \textsc{LLaMA-2-7B}.}
\caption{Debiasing methods on \our.
All rows are evaluated on the fixed $n\!=\!500$ subsample; vanilla rows re-aggregate the full-set baselines of Table~\ref{tab:baseline} on this subsample (Appendix~\ref{app:exp-setup-details}).
\textbf{Bold}: best per column within each model block ($\uparrow$ for $\mathrm{Coverage}$, $\downarrow$ for the others).
RLHF is applied only to \textsc{LLaMA-2-7B}.}
\label{tab:debias}
\end{table}

%\paragraph{No debiasing method strictly Pareto-improves over vanilla.}
%Every variant in Table~\ref{tab:debias} reduces $\mathrm{Coverage}$ relative to its vanilla baseline.
%Three of the seven configurations (LLaMA-RLHF, LLaMA-DPO, Qwen-DPO) further \emph{increase} per-stance leakage on \emph{every} stance, and the remaining four improve $\mathrm{SBias}^{k}$ on at most two of the three stances.
%The debiased points slide from vanilla's (high-Coverage, high-bias) corner toward (lower-Coverage, lower-bias) without entering the desired (high-Coverage, low-bias) regime.
%$\mathrm{BiasRatio}$ alone would have suggested all four methods work; reading $\mathrm{BiasRatio}$ together with $\mathrm{Coverage}$ and the per-stance $\mathrm{SBias}^{k}$ shows that what they primarily do is shrink the output---exactly the suppression failure mode we diagnosed for \textsc{LLaMA-2-7B} vanilla.

\paragraph{Mitigation lowers bias density mainly by reducing coverage.}
Table~\ref{tab:debias} shows that every debiasing method reduces $\mathrm{Coverage}$ relative to vanilla. Although $\mathrm{BiasRatio}$ also decreases in most cases, per-stance $\mathrm{SBias}^{k}$ often changes little or worsens. Four configurations---LLaMA-DS, LLaMA-RLHF, LLaMA-DPO, and Qwen-DPO---increase leakage on all three stances; only Qwen-BLE lowers leakage on all three, and the remaining two configurations improve at most two stances.

%\paragraph{Prompt-side and alignment-side methods sit at distinct operating points.}
%Reading Table~\ref{tab:debias} as displacement from each vanilla baseline (also visualized as arrows in Appendix~\ref{app:debias-arrows-fig}, Figure~\ref{fig:debias-arrows}):
%BLE and DS produce short displacements---$\mathrm{Coverage}$ drops $3.9$--$13.7$~pp and $\mathrm{BiasRatio}$ drops $0.6$--$3.5$~pp, a low-risk-low-reward regime.
%RLHF on \textsc{LLaMA-2-7B} sits between prompt-side and DPO, trading $-7.1$~pp $\mathrm{Coverage}$ for $-1.1$~pp $\mathrm{BiasRatio}$.
%DPO is qualitatively different: for both models it slashes $\mathrm{BiasRatio}$ to a third of its vanilla value but also slashes $\mathrm{Coverage}$ by $24.7$~pp (\textsc{LLaMA}) and $35.9$~pp (\textsc{Qwen}).
%We interpret DPO under bias-graded preference pairs as collapsing the model toward a ``say less, say neutral'' regime: the policy reduces overall propositional content, which mechanically reduces both biased and unbiased atomic facts.
%This pattern is consistent with the suppression mechanism diagnosed for \textsc{LLaMA-2-7B} vanilla; the joint reporting framework distinguishes the two only when $\mathrm{Coverage}$ and per-stance $\mathrm{SBias}^{k}$ are read together.

\paragraph{Prompting is mild, while DPO induces strong output suppression.}
BLE and DS produce modest shifts: $\mathrm{Coverage}$ drops by $1.0$--$11.2$~pp and $\mathrm{BiasRatio}$ by $0.9$--$3.3$~pp (displacements visualized in Appendix~\ref{app:debias-arrows-fig}). RLHF on \textsc{LLaMA-2-7B} lies between prompting and DPO ($-4.3$~pp $\mathrm{Coverage}$). DPO is much stronger: it reduces $\mathrm{BiasRatio}$ to a third (\textsc{LLaMA}) and a quarter (\textsc{Qwen}) of the vanilla value, but also cuts $\mathrm{Coverage}$ by $21.9$~pp on \textsc{LLaMA} and $33.4$~pp on \textsc{Qwen}. This suggests a ``say less, say neutral'' failure mode, where biased facts decrease because the model produces substantially fewer facts overall.

%\paragraph{\textsc{Qwen2-7B} is more sensitive to prompt-side intervention than \textsc{LLaMA-2-7B}.}
%BLE and DS reduce \textsc{Qwen2-7B}'s $\mathrm{Coverage}$ by $11.7$ and $13.7$~pp respectively, against only $3.9$~pp for \textsc{LLaMA-2-7B}, while per-stance $\mathrm{SBias}^{k}$ moves correspondingly less.
%A plausible explanation is that \textsc{Qwen2-7B}'s vanilla $\mathrm{Coverage}$ is substantially higher ($.565$ vs.\ $.476$), leaving more headroom to lose under conservative instructions; whether this generalizes to other high-$\mathrm{Coverage}$ models is left to future work.

\paragraph{\textsc{Qwen2-7B} is more sensitive to prompt-side intervention.}
BLE and DS reduce \textsc{Qwen2-7B}'s $\mathrm{Coverage}$ by $9.2$ and $11.2$~pp, compared with about $1$~pp for \textsc{LLaMA-2-7B}. A likely reason is that \textsc{Qwen2-7B} starts from a higher-coverage vanilla answer ($.540$ vs.\ $.447$), leaving more content to suppress under conservative instructions.

%\paragraph{Finding.}
%For \textbf{RQ3}, none of the four mitigation strategies we tested effectively reduce informational bias on \our.
%Across all four methods, the dominant effect is output shrinkage rather than selective bias filtering---$\mathrm{Coverage}$ falls, $\mathrm{BiasRatio}$ falls in tandem, and the per-stance $\mathrm{SBias}^{k}$ (each invariant to output length) change only marginally and on several stances in the wrong direction.
%This pattern is robust across two model families, two intervention regimes (prompt-side and alignment-side), and a $36$~pp range of intervention strength, suggesting that current debiasing techniques are not well calibrated for the partisan-stance setting that \our defines and motivating the discussion of more targeted training objectives in Section~\ref{sec:conclusion}.

\paragraph{Takeaway.}
For \textbf{RQ3}, the tested mitigation strategies do not effectively reduce informational bias on \our. Their dominant effect is output shrinkage: $\mathrm{Coverage}$ falls, $\mathrm{BiasRatio}$ falls partly as a consequence, and $\mathrm{SBias}^{k}$ remains stable or worsens on several stances. This pattern holds across model families and intervention types, suggesting that common debiasing methods are not well calibrated for stance-specific informational bias in RAG-based QA.

\subsection{Robustness under Noisy Context}
\label{sec:exp-noisy}

%The vanilla setting fixes the evidence to the curated triplet from AllSides.
%In a deployment-faithful setting, however, a retriever may surface chunks that are topically related to $\mathcal{Q}$ but originate outside that triplet.
%We test whether the metric framework remains stable, and whether bias inheritance is sensitive, under such heterogeneous evidence.

In real deployments, a retriever may surface topically related content beyond the curated AllSides triplet; we therefore test whether the main metric patterns remain stable under such uncurated off-triplet evidence.

%\paragraph{Noisy-context construction.}
%For each question we (i)~issue $\mathcal{Q}$ as a DuckDuckGo query and scrape up to ten top-ranked URLs with a headless browser;
%(ii)~segment the scraped pages and the original triplet articles into 2{,}048-character chunks;
%(iii)~apply a two-stage retriever (BM25 top-20, then dense reranking with \textsc{all-MiniLM-L6-v2}) to select the single most relevant chunk; and
%(iv)~prepend this chunk as a fourth, unlabeled evidence piece to the standard $(c_l,c_c,c_r)$ prompt, leaving everything else identical.
%We do \emph{not} control or verify the stance of the retrieved chunk---it is simply topically-related open-web content outside the curated triplet---so this setting probes robustness to \emph{uncurated} additional evidence rather than a clean stance.
\paragraph{Noisy-context construction.}
For each question, we issue $\mathcal{Q}$ as a DuckDuckGo query and scrape up to ten top-ranked URLs. We segment both the scraped pages and the original triplet articles into 2{,}048-character chunks, retrieve BM25 top-20 chunks, rerank them with \textsc{all-MiniLM-L6-v2}, and prepend the highest-ranked off-triplet chunk as a fourth, unlabeled evidence piece to the standard evidence triplet $\mathcal{D}=\{D^{L},D^{C},D^{R}\}$. We do not verify the stance or factuality of this retrieved chunk.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\scalebox{0.78}{
\begin{tabular}{@{}l c c c c c@{}}
\toprule
\textbf{Setting} & $\mathrm{Cov.}\uparrow$ & $\mathrm{BR}\downarrow$
& $\mathrm{SB}^{L}\downarrow$ & $\mathrm{SB}^{R}\downarrow$ & $\mathrm{SB}^{C}\downarrow$ \\
\midrule
\textsc{LLaMA-2-7B}        & .447 & .079 & .512 & .579 & .517 \\
\quad +noisy ctx           & .455 & .066 & .497 & .516 & .489 \\
$\Delta$ (pp)              & $+0.7$ & $-1.3$ & $-1.5$ & $-6.4$ & $-2.8$ \\
\midrule
\textsc{Qwen2-7B}          & .540 & .100 & .598 & .596 & .610 \\
\quad +noisy ctx           & .504 & .092 & .582 & .585 & .550 \\
$\Delta$ (pp)              & $-3.6$ & $-0.8$ & $-1.7$ & $-1.1$ & $-6.0$ \\
\bottomrule
\end{tabular}}
%\caption{Effect of injecting one retrieved off-triplet chunk into the evidence ($n\!=\!500$).
%Vanilla rows are repeated from Appendix~\ref{app:vanilla-numbers} (Table~\ref{tab:baseline}) for the $\Delta$ computation, expressed in percentage points.
%For both models, $\mathrm{Coverage}$ and $\mathrm{BiasRatio}$ move in the same direction (downward), and the within-model ordering of $\mathrm{SBias}^{l/r/c}$ is preserved.}
\caption{Effect of adding one off-triplet retrieved chunk ($n\!=\!500$). Vanilla rows re-aggregate the baselines on the same subsample; deltas are in percentage points, computed from unrounded values.}
\label{tab:noisy}
\end{table}

%\paragraph{Off-triplet evidence dilutes both $\bm{\mathrm{Coverage}}$ and $\bm{\mathrm{BiasRatio}}$.}
%For both \textsc{LLaMA-2-7B} and \textsc{Qwen2-7B}, the additional chunk pushes $\mathrm{Coverage}$ down by $2.1$ and $6.1$~pp respectively (Table~\ref{tab:noisy}).
%$\mathrm{BiasRatio}$ also decreases by a comparable $1.0$~pp for both models, and the per-stance bias-retention rates $\mathrm{SBias}^{k}$ all decline.
%The most consistent reading is mechanical: the noisy chunk crowds out triplet-grounded propositions in the all-sides answer ($\mathrm{Coverage}\!\downarrow$) and adds off-triplet content that dilutes the share of triplet-derived bias facts in the output ($\mathrm{BiasRatio}\!\downarrow$).
%The asymmetric magnitude---\textsc{Qwen2-7B}'s $\mathrm{Coverage}$ drops three times more than \textsc{LLaMA-2-7B}'s---is consistent with \textsc{Qwen2-7B} producing longer, more triplet-grounded vanilla outputs that have more to lose.

\paragraph{Off-triplet evidence dilutes bias density more than coverage.}
Table~\ref{tab:noisy} shows that adding one noisy chunk leaves $\mathrm{Coverage}$ essentially flat for \textsc{LLaMA-2-7B} ($+0.7$~pp) and lowers it by $3.6$~pp for \textsc{Qwen2-7B}, while $\mathrm{BiasRatio}$ drops for both ($-1.3$ and $-0.8$~pp) and every per-stance $\mathrm{SBias}^{k}$ declines. This pattern is consistent with dilution: the off-triplet chunk displaces stance-specific biased content more than shared content. The larger coverage drop for \textsc{Qwen2-7B} is consistent with its higher-coverage vanilla answers, which leave more triplet-grounded content to displace.

%\paragraph{Stance asymmetry of selective bias is preserved under noise.}
%A natural concern with off-triplet evidence is that it could swap the relative ordering of stance-conditional leakage.
%This does not happen: within each model, $\mathrm{SBias}^{r}\!>\!\mathrm{SBias}^{l}$ and $\mathrm{SBias}^{l}\!>\!\mathrm{SBias}^{c}$ (or $\mathrm{SBias}^{r}\!>\!\mathrm{SBias}^{c}$) still hold under the noisy setting, mirroring Figure~\ref{fig:sbias_vanilla}.
%The structural finding that center bias is least amplified is therefore not an artifact of the controlled triplet setup but a property the framework detects under deployment-like evidence as well.

\paragraph{Leakage declines on every stance.}
Noise lowers per-stance leakage across the board and does not inflate any stance: under the noisy setting, center-aligned biased facts are the least amplified for both models, with the largest reductions on the right side for \textsc{LLaMA-2-7B} ($-6.4$~pp) and the center side for \textsc{Qwen2-7B} ($-6.0$~pp).


%\paragraph{Finding.}
%Noisy off-triplet context attenuates the metrics uniformly without redirecting them: signs of all $\Delta$ are negative, and the stance-asymmetry signal is preserved.
%We treat this as evidence that our framework measures a stable, evidence-driven property of $\mathcal{A}_{\text{all}}$ rather than an artifact of curated triplets.
\paragraph{Takeaway.}
Noisy off-triplet context lowers bias density and per-stance leakage while leaving coverage flat or lower, without inflating leakage on any stance. The framework's signals thus remain measurable under deployment-like evidence rather than being an artifact of curated article triplets.

\subsection{Scale and Recency}
\label{sec:exp-scale}

A natural concern is that the pool above under-represents newer or larger models. Simply adding one newer and larger model would not settle it: contrasting \textsc{Qwen2-7B} with \textsc{Qwen3-32B}, for instance, varies generation and parameter count jointly, so neither factor can be isolated. We therefore extend the evaluation along two \emph{paired} axes instead. The \emph{scale} axis holds family and generation fixed and increases parameters by $\sim$$10\times$ (\textsc{Qwen2.5-7B}$\,\to\,$\textsc{Qwen2.5-72B}; \textsc{Llama-3.1-8B}$\,\to\,$\textsc{Llama-3.1-70B}); the \emph{recency} axis holds size approximately fixed and moves one generation forward (\textsc{Qwen2-7B}$\,\to\,$\textsc{Qwen3-8B}; \textsc{LLaMA-2-7B}$\,\to\,$\textsc{Llama-3.1-8B}). Each pair therefore varies one factor at a time. \textsc{Qwen3-32B} is reported alongside them as a single larger, newer data point rather than as a controlled contrast. The six additional models are scored with the unchanged pipeline, including the same \textsc{Gemma-3-27B-it} decomposer and reference landscape. Table~\ref{tab:scale-recency} reports all rows on the fixed $n\!=\!500$ subsample of Sections~\ref{sec:exp-debias} and~\ref{sec:exp-noisy}, with the two pool baselines re-aggregated on the same subsample; because $\mathrm{Coverage}$ comparisons are sensitive to answer length, we also report mean words per answer.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.69}{
\begin{tabular}{@{}l c c c ccc c@{}}
\toprule
\textbf{Model} & \textbf{Year} & $\mathrm{Cov.}\!\uparrow$ & $\mathrm{BR}\!\downarrow$
& $\mathrm{SB}^{L}\!\downarrow$ & $\mathrm{SB}^{R}\!\downarrow$ & $\mathrm{SB}^{C}\!\downarrow$ & \textbf{Words} \\
\midrule
\multicolumn{8}{@{}l}{\emph{Qwen family}} \\
\textsc{Qwen2-7B}      & 2024 & .540 & .100 & .598 & .596 & .610 & 93.7  \\
\textsc{Qwen2.5-7B}    & 2024 & .387 & .115 & .463 & .558 & .530 & 72.5  \\
\textsc{Qwen2.5-72B}   & 2024 & .373 & .090 & .543 & .617 & .656 & 97.1  \\
\textsc{Qwen3-8B}      & 2025 & .378 & .100 & .551 & .582 & .640 & 85.2  \\
\textsc{Qwen3-32B}     & 2025 & .350 & .100 & .508 & .635 & .651 & 92.8  \\
\midrule
\multicolumn{8}{@{}l}{\emph{Llama family}} \\
\textsc{LLaMA-2-7B}    & 2023 & .447 & .079 & .512 & .579 & .517 & 125.1 \\
\textsc{Llama-3.1-8B}  & 2024 & .359 & .118 & .411 & .457 & .474 & 64.2  \\
\textsc{Llama-3.1-70B} & 2024 & .379 & .120 & .463 & .539 & .505 & 75.0  \\
\bottomrule
\end{tabular}}
\caption{Scale and recency on the fixed $n\!=\!500$ subsample.
The \textsc{Qwen2-7B} and \textsc{LLaMA-2-7B} rows re-aggregate the vanilla pool baselines on this subsample and therefore differ slightly from the full-set values in Table~\ref{tab:baseline}; the six additional models are scored with the unchanged pipeline.
\textbf{Words}: mean words per answer, reported because $\mathrm{Coverage}$ comparisons are length-sensitive. In-text differences are computed from unrounded values.}
\label{tab:scale-recency}
\end{table}

\paragraph{Bias density does not improve with recency or scale.}
$\mathrm{BiasRatio}$ is a per-fact density and hence robust to answer length, and it stays within a narrow $.079$--$.120$ band across all eight models. Neither generational pair lowers it: the Qwen pair is exactly flat ($.100\!\to\!.100$), and the Llama pair \emph{rises} by $3.9$~pp ($.079\!\to\!.118$) even though the newer model produces answers half as long. Within-family scaling leaves it flat for Llama-3.1 ($.118\!\to\!.120$), and the modest $-2.5$~pp drop for \textsc{Qwen2.5-72B} is accompanied by sharply higher stance-selective leakage.

\paragraph{Scaling raises stance-selective leakage in both families.}
The $\sim$$10\times$ within-family pairs leave $\mathrm{Coverage}$ essentially unchanged ($-1.4$~pp for Qwen2.5, $+2.1$~pp for Llama-3.1) while raising \emph{all three} $\mathrm{SBias}^{k}$ scores: $+7.9$/$+5.8$/$+12.5$~pp ($L$/$R$/$C$) for \textsc{Qwen2.5-7B}$\,\to\,$\textsc{Qwen2.5-72B} and $+5.1$/$+8.2$/$+3.1$~pp for \textsc{Llama-3.1-8B}$\,\to\,$\textsc{Llama-3.1-70B}. \textsc{Qwen2.5-72B} also produces $34\%$ longer answers than its 7B sibling without gaining coverage, and posts the highest center-side leakage in the extended pool ($\mathrm{SBias}^{C}\!=\!.656$): the additional capacity is spent reproducing stance-specific biased facts rather than balancing shared information. Notably, the center under-amplification observed in the main pool weakens here: for several 2024--2025 models, $\mathrm{SBias}^{C}$ is the largest of the three sides, so the relative protection of center-aligned facts should not be assumed to persist across generations.

\paragraph{Coverage comparisons require the length column.}
The 2024--2025 models answer more concisely ($64$--$97$ words versus $94$--$125$ for the earlier pool), and their $\mathrm{Coverage}$ values are correspondingly lower ($.350$--$.387$). \textsc{Qwen3-32B} is the clearest case: it matches \textsc{Qwen2-7B} in words per answer ($92.8$ vs.\ $93.7$) and atomic facts per answer ($19.5$ vs.\ $21.8$), yet covers $19$~pp less. The Llama generational pair halves its answer length ($125\!\to\!64$ words), so its $8.9$~pp coverage drop partly reflects brevity; the Qwen generational pair, in contrast, loses $16.2$~pp of coverage with only $9\%$ fewer words. Length does not explain everything---\textsc{Qwen2.5-72B} writes the longest answers in its family yet covers no more---but cross-generation coverage contrasts should be read jointly with answer length, whereas the per-fact $\mathrm{BiasRatio}$ and $\mathrm{SBias}^{k}$ findings above are length-robust.

\paragraph{Takeaway.}
Neither moving to a newer generation nor scaling $\sim$$10\times$ within a family moves models toward the desired high-coverage, low-bias regime: bias density never leaves the vanilla band, and scaling increases leakage on every stance in both families. The informational-bias patterns measured by \our are therefore not artifacts of evaluating older or smaller models.

